Phasic Self-Imitative Reduction for Sparse-Reward Goal-Conditioned Reinforcement Learning

It has been a recent trend to leverage the power of supervised learning (SL) towards more effective reinforcement learning (RL) methods. We propose a novel phasic approach by alternating online RL and offline SL for tackling sparse-reward goal-conditioned problems. In the online phase, we perform RL training and collect rollout data while in the offline phase, we perform SL on those successful trajectories from the dataset. To further improve sample efficiency, we adopt additional techniques in the online phase including task reduction to generate more feasible trajectories and a value-difference-based intrinsic reward to alleviate the sparse-reward issue. We call this overall algorithm, PhAsic self-Imitative Reduction (PAIR). PAIR substantially outperforms both non-phasic RL and phasic SL baselines on sparse-reward goal-conditioned robotic control problems, including a challenging stacking task. PAIR is the first RL method that learns to stack 6 cubes with only 0/1 success rewards from scratch.

==> 41offline.tex <==
\subsection{Collecting dataset for offline learning}
\yf{Describe data collection in a new section??}
The offline phase aims to improve policy using a fixed transition dataset $\mathcal{B}$ generated from the agent's rollout trajectories in the previous online phase. 
% We first describe how the dataset is constructed before each offline training phase. 
The successful trajectories are directed inserted into $\mathcal{B}$ as is done in SIL~\cite{oh2018self}. 
For original unsuccessful trajectories, we can apply task reduction on their initial states and goals to search for intermediate states, and re-execute the current policy along the decomposed two sub-tasks. If both sub-tasks are accomplished, we relabel the two sub-trajectories as a successful demonstration for the original task, and restore it into $\mathcal{B}$ as well. In this way, task reduction incorporates compositionality into the data, and we empirically find it boosting the performance on very complex compositional problems.
Following the common practice in continuous multi-task goal-conditioned RL~\cite{andrychowicz2017hindsight,ghosh2020learning,kalashnikov2021mt}, we also convert the failed trajectories into artificial successful ones by relabeling their goals, which further enriches supervision signal from rollout data. 

\subsection{Learning from batch data in offline phase}
We propose to decouple SL objective from RL, and perform offline policy improvement in a separate phase.
Given the dataset $\mathcal{B}$ that contains only successful trajectories, any state-of-the-art imitation learning or offline RL algorithms can be applied in this phase to improve the policy performance. 
We by default optimize a weighted behavior cloning objective $\mathcal{L}^{SL}$ in this phase, which is simple but effective to distill information from $\mathcal{B}$ to the policy. We also experiment with a representative offline RL algorithm Desicion Transformer~\cite{chen2021decision} and find it also compatible with our pipeline. \yf{still not sure if AWAC can work in at least one domain..}

Note that we do not optimize SL objective as an auxiliary loss along with online RL training. The intuition is that joint optimization of multiple objectives may suffer from interference between different objectives, which is similar to the intuition of phasic training in PPG~\cite{cobbe21ppg}. \yw{These texts should be put into appendix!} \yf{The practical reason is that we can more easily apply different hyperparameters (e.g., batch size) to offline and online training to get better performance.} \yw{put these into intro!} We empirically verify that SL and RL in separate phases leads to better sample efficiency than jointly optimizing them in a single phase.\yf{refer to expr.} 

==> 42online.tex <==
\subsection{Policy improvement in online phase}
The policy trained in the offline phase may not be perfect to handle all possible tasks since offline data amount and coverage is always limited in practice.   
In order to further improve its performance, we allow it to perform ordinary RL training by trial-and-error in the environment. We choose PPO~\cite{schulman17ppo} as the default online RL algorithm since it is generally applicable to various domains and easy to tune. \yf{DT actually also uses PPO objective in online phase. Should we say DT or PPO here?} In the same time, we can collect a bunch of new data for the next training phase. 

==> 44enhance.tex <==
\textbf{Practical enhancement: } 
We find a value-based intrinsic reward useful to alleviate the sparse reward issue. Specifically, we use the temporal difference of the learning value function as an intrinsic reward, and add it to the original 0-1 reward:
\begin{align*}
    & r^{\textrm{d}}(s_t, a_t, g) = r(s_t, a_t, g) + \alpha \Delta V, \\
    & \Delta V = V(s_{t+1}, a_{t+1}, g) - V(s_t, a_t, g).
\end{align*}
The dense reward $r^{\textrm{d}}$ is then used in RL training. \yf{add some discussion?}

\yf{relation to AWAC?}
